Multiple phoretic mechanisms in the self-propulsion of a Pt-insulator Janus swimmer

We present a detailed theoretical study which demonstrates that electrokinetic effects can also play a role in the motion of metallic-insulator spherical Janus particles. Essential to our analysis is the identification of the fact that the reaction rates depend on Pt- coating thickness and that the thickness of coating varies from pole to equator of the coated hemisphere. We find that their motion is due to a combination of neutral and ionic diffusiophoretic as well as electrophoretic effects whose interplay can be changed by varying the ionic properties of the fluid. This has great potential significance for optimising performance of designed synthetic swimmers.

==> reaction_kinetics.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reaction kinetics}\label{appA}
%
In this section, our goal is to obtain the fluxes on the surface of the swimmer,  $\bar{\mathcal{J}}_i$ of all the chemical species involved in the H$_2$O$_2$ decomposition
\begin{equation}
\mbox{Pt} +  2{\text{H}_2\text{O}_2} \ \rightarrow \boxed{\textsf{Intermediate complexes}} \rightarrow \ \mbox{Pt} + 2\text{H}_2\text{O} + \text{O}_2 \ . \label{h2o2:decomp:generic:app}
\end{equation} 
Though a complete picture of the intermediate complexes in reaction (\ref{h2o2:decomp:generic:app}) remains elusive, it is known that there are neutral pathways as well as ionic electrochemical pathways~\cite{mckee1969catalytic,bianchi1962catalytic,katsounaros2012hydrogen}. 
\yhy{Therefore, we consider below two possible reaction schemes involving both neutral as well as electroneutral pathways}.
%

\subsection{Reaction scheme 1}
First, we consider a reaction scheme for the reaction (\ref{h2o2:decomp:generic:app}) made up of two pathways, one neutral 
% taking into account both the inert chemical pathway
\begin{equation}
\mbox{Pt} +  2{\text{H}_2\text{O}_2} \ \overset{k_0}{\longrightarrow} \ \mbox{Pt}\left({\text{H}_2\text{O}_2} \right)  + {\text{H}_2\text{O}_2} \ \overset{k_1}{\rightarrow }\ \mbox{Pt}\left({\text{H}_2\text{O}_2} \right)_2 \ \overset{k_2}{\rightarrow} \  \mbox{Pt} + 2\text{H}_2\text{O} + \text{O}_2 \ ,  \label{h2o2:decomp:neutral}
\end{equation} 
and the other ionic involving charged intermediates,
%and an electrochemical pathway involving charged intermediates
\begin{align}
\mbox{Pt} +  2{\text{H}_2\text{O}} \quad  \underset{k_{-3}}{\overset{k_3}{\rightleftharpoons}} \quad \mbox{Pt}\left({\text{H}_2\text{O}_2} \right) + 2e^-  + 2\text{H}^+ \ . \label{h2o2:decomp:charged}
\end{align} 
%In addition, water naturally dissociate into protons and hydroxide ions
%\begin{equation}
%{\text{H}_2\text{O}} \ \rightleftharpoons \ 2\text{H}^+ + \text{OH}^-.
%\end{equation}
%
The reaction scheme above and the intermediate states denoted by $(0,1,2)$ are enumerated in Fig. (\ref{reaction_scheme}).
\begin{figure}
\begin{center}
\includegraphics[scale=.4]{reaction_schematic1}
\end{center}
\caption{(\textbf{Reaction scheme 1}): Schematic complexation kinetics of the Platinum catalyst with free ($0$'th state) Pt occupied with probability density $p_0$; first complex state $\text{Pt}(\text{H}_2\text{O}_2)$ occupied with probability density $p_1$, and the second complex state $\text{Pt}(\text{H}_2\text{O}_2)_2$ occupied with probability density $p_2$.} 
\label{reaction_scheme}
\end{figure}
The kinetics of the Pt catalyst complexation in stationary state reads
\begin{align}  
0 & = \partial_t p_0 = -\  k_0  \bar{c}_{hp} \ p_0 - k_3 \ p_0 + k_2 \ p_2  + k_{-3} \bar{c}_h^2 \ p_1 \ , \\
0 & = \partial_t p_1 =   \quad k_0  \bar{c}_{hp} \ p_0 + k_3 \ p_0 - k_1 \bar{c}_{hp} \ p_1  - k_{-3}  \bar{c}_h^2 \ p_1  \  , \\
0 & = \partial_t p_2 = \quad k_1  \bar{c}_{hp} \ p_1 - k_2  \ p_2 \  , \label{probability:kinetics:inhomogeneous} 
\end{align}
where $p_i$'s are the complexation probabilities. Solving for these probabilities $p_i$, we obtain
\begin{align}
p_0 & = \mathcal{M}^{-1} k_2 \left( k_1 \bar{c}_{hp} + k_{-3} \bar{c}_h^2  \right)  \  ,  \\
p_1 & = \mathcal{M}^{-1} k_2 \left( k_0 \bar{c}_{hp} + k_3 \right)  \ ,   \\
p_2 & = \mathcal{M}^{-1} k_1 \bar{c}_{hp} \left( k_0  \bar{c}_{hp} + k_3  \right)  \ , 
\end{align}
where the normalization condition $p_0+p_1+p_2=1$ was used and we have defined
\begin{equation}
\mathcal{M} := k_2 k_3 + k_2 k_{-3}  \bar{c}_h^2 +  \left( k_0 k_2 + k_1 k_3 + k_1 k_2 \right)  \bar{c}_{hp} + k_0 k_1  \bar{c}_{hp}^2   \ .
\end{equation}
This  leads to expressions for the fluxes $\bar{\mathcal{J}}_i$ of $i \in \{o,hp,h\}$
\begin{align}
 \bar{\mathcal{J}}_o(\theta)   &= \quad k_2 \ p_2 K(\cos \theta) \ , \nonumber \\
 &  =  \mathcal{M}^{-1} k_1 k_2 \bar{c}_{hp} \Big( k_0  \bar{c}_{hp} + k_3  \Big) K(\cos\theta) \ , \label{o2:flux} \\
 \bar{\mathcal{J}}_{hp}(\theta)&=  -  \left( k_0 \ p_0 + k_1 \ p_1  \right) \bar{c}_{hp}  K(\cos \theta) \ , \nonumber  \\
 & = -  \mathcal{M}^{-1} k_2\bar{c}_{hp} \Big( k_1k_3 + k_0k_{-3}\bar{c}_h^2 + 2 k_0k_1\bar{c}_{hp}  \Big) K(\cos\theta) \ , \label{hp:flux}  \\
\bar{\mathcal{J}}_{h}(\theta)  &=  2 \ \left( k_3 \ p_0 - k_{-3} \bar{c}_h^2 \ p_1  \right)  K(\cos \theta)  \ , \nonumber  \\
& = 4 \mathcal{M}^{-1} k_2 \bar{c}_{hp} \Big( k_1k_3 - k_0k_{-3} \bar{c}_h^2 \Big) K(\cos\theta) \ ,  \label{h:flux}
\end{align} 
and for the fluxes of hydroxide and the salt, $\bar{\mathcal{J}}_{oh} = 0, \bar{\mathcal{J}}_{s,\pm} = 0$. Measurements of the reaction rates~\cite{ebbens2014electrokinetic} imply that $\bar{\mathcal{J}}_{hp}$ and $\bar{\mathcal{J}}_o$ vary with the Pt coating thickness (of $\sim$nm scale). Hence we may assume that the rate `constants' $k_i$'s vary in a similar manner.    \\

{Since the thickness of the coating varies across the Pt cap,  the reaction rates  $k_i(\theta)$'s vary over the coated hemisphere, and can be expanded in Legendre polynomials. We consider a simple linear approximation
\begin{equation}
k_i(\theta) \cong k_i^{(0)} + k_i^{(1)} \cos \theta \  ,
\end{equation}
in $\cos\theta$ and we assume weak variation $k_i^{(1)}/k_i^{(0)} \ll 1$ of the rates.}  \\


%(\emph{Proton flux})  
{The solute fluxes $\bar{\mathcal{J}}_i$ above in eqns. (\ref{o2:flux} - \ref{h:flux}) require the inner (Debye-layer) proton concentration profile
\begin{equation}
\bar{c}_h(1,\theta)/c_h^{\infty} =  \left( 1 + C_h(1,\theta) \right) e^{- \zeta(\theta)} \ ;  \qquad  \zeta(\theta) = \varphi_s -  \Phi(1,\theta) \ ,
\end{equation}
from eqn. (\ref{inner:outer:relation}) in Appendix \ref{app:slip:velocity:derivations}, where $C_h(1,\theta)$ and $\Phi(1,\theta)$ are the deviations from the uniform background of proton concentration and electric fields. $\varphi_s$ is the electric potential on the   swimmer surface. Hence, the proton flux at the outer edge of the double-layer reads
\begin{equation}
\bar{\mathcal{J}}_h ( \theta ) =  4 \mathcal{M}^{-1} k_2 \bar{c}_{hp} \  \left( k_1 k_3 - k_0 k_{-3} \left(c_h^{\infty}\right)^2 (1+C_h)^2 e^{- 2 \zeta(\theta) }\right)  K(\cos \theta) \  .
\end{equation} }

{Furthermore, Taylor-expanding the flux up to linear order in $k_i^{(1)}$, and the deviations $C_h, \ \Phi$ ;
\begin{equation} 
\bar{\mathcal{J}_h} (\theta) = \left( \bar{\mathcal{J}}_h^{(0)}  \ + \ \bar{\mathcal{J}}_h^{(1)} \ P_1(\cos \theta)  + \ \bar{\mathcal{J}}_h^{'(0)} \  \left(\Phi + C_h \right)  \right) K(\cos\theta)   %+  \mathcal{O}\left(\frac{ \bar{\mathcal{J}}_h^{(j)} \mathcal{M}^{(1)}}{\mathcal{M}^{(0)}}\right) 
\ , \label{H:flux:approx0}
\end{equation} 
where $j= \{ 0,1,2\}$. We define 
\begin{align}
\bar{\mathcal{J}}_h^{(0)} & =  4  \{ k_2 c_{hp} \}^{(0)} \ \left( \{k_1k_3\}^{(0)} - \{k_0k_{-3}\}^{(0)} (c_h^{\infty})^2 e^{-2 \varphi_s } \right)/\mathcal{M}^{(0)} \ ,  \label{H:flux:0} 
 \\
\bar{\mathcal{J}}_h^{(1)} & =  4 \{ k_2 c_{hp} \}^{(0)} \ \left( \{k_1k_3\}^{(1)} - \{k_0k_{-3}\}^{(1)} (c_h^{\infty})^2 e^{-2 \varphi_s  } \right) / \mathcal{M}^{(0)} \ ,
\label{H:flux:1}  
\\
\bar{\mathcal{J}}_h^{'(0)} & =  8 \{ k_2 c_{hp} \}^{(0)} \{k_0k_{-3}\}^{(0)} (c_h^{\infty})^2 e^{-2 \varphi_s }  / \mathcal{M}^{(0)} \ , \label{H:flux:2}  \\
\mathcal{M}^{(0)} & = \left \{ k_2 k_3 + k_2 k_{-3}  \bar{c}_h^2 +  \left( k_0 k_2 + k_1 k_3 + k_1 k_2 \right)  \bar{c}_{hp} + k_0 k_1  \bar{c}_{hp}^2 \right\}^{(0)}  \ . 
\end{align} 
Now, imposing net charge conservation, equation (\ref{quasi:steady:constraint}) on the swimmer surface,  equation (\ref{H:flux:approx0}) for the proton flux leads to 
\begin{equation}
\bar{\mathcal{J}}_h^{(0)} + \frac{1}{2} \bar{\mathcal{J}}_h^{(1)} + \bar{\mathcal{J}}_h^{'(0)} \int_0^{\pi}  \left( \Phi + C_h\right)  K(\cos \theta) \ \sin \theta \ d \theta  = 0 \ .
\end{equation}
Then, substituting for $\bar{\mathcal{J}}_h^{(i)}$'s (from eqns. \ref{H:flux:0}-\ref{H:flux:2}) and simplifying ;
\begin{align}  
    (c_h^{\infty})^2 e^{-2 \varphi_s }  \   &  \left(   1 + \frac{1}{2} \frac{ \{k_0k_{-3}\}^{(1)}}{\{k_0k_{-3}\}^{(0)} }    +  2  \int_0^{\pi} \left( \Phi + C_h \right)K(\cos\theta) \sin\theta \, d\theta  \right)   \\
   &\qquad \qquad\qquad \qquad \qquad  \qquad  = \quad   \frac{\{k_1k_{3}\}^{(0)}}{\{k_0k_{-3}\}^{(0)} }    + \frac{1}{2}  \frac{\{k_1k_{3}\}^{(1)}}{\{k_0k_{-3}\}^{(0)} }    \     . 
\end{align} 
%
For a uniform coating (i.e $k_i^{(1)} = 0$ for all $i$'s), which has the trivial solution $\Phi = C_h =  0$, the zero total current condition gives rise to 
% Remember, we are expanding about the reference uniform catalyst coating surface state (i.e $k_i^{(1)} = 0$ for all $i$'s); which has the trivial 
% solution $\Phi = C_h =  0$ . This implies that to the leading linear order of our expansion, the steady state constraint of vanishing 
%(surface average) proton current is satisfied by
\begin{align}  
  (c_h^{\infty})^2 e^{-2 \varphi_s }  \   \cong  \    \frac{\{k_1k_{3}\}^{(0)}}{\{k_0k_{-3}\}^{(0)} }    \   .   \label{H:balance}
\end{align} 
which is all that is required for a linear expansion about a uniform coating.
%
%
%
Hence solving for the swimmer potential $\varphi_s$, we obtain the equation 
\begin{equation}
\varphi_s  = \varphi_s^{\ominus} - \ln 10 \ \mbox{pH} \ , \label{zeta:potential:equilibrium}
\end{equation}
where $\mbox{pH} = - \log_{10} c_h^{\infty}$ (with $c_h^{\infty}$ measured in molar units) and 
%the kinetically defined potential
\begin{equation}
 \varphi_s^{\ominus} =  - \frac{1}{2}  \ln \left(  \frac{ \{ k_1 k_3 \}^{(0)}  }{  \{ k_0 k_{-3} \}^{(0)} } \right) \ .
\end{equation} 
Therefore, eliminating the swimmer potential and proton background concentration ($\varphi_s, \, c_h^{\infty}$) by substituting eqn. (\ref{H:balance}) into eqn. (\ref{H:flux:approx0}) and keeping only linear perturbations, the proton flux assumes a simple form
\begin{equation} \boxed{
\bar{\mathcal{J}}_h(\theta)  \cong \left[ \Delta k_{\text{eff}}^{(h)} \  \left( 1 - 2 \cos \theta \right)   - k_{\text{eff}}^{(h)} \ \delta \left(\Phi + C_h \right) \right] c_{hp}^{\infty} \  K(\cos \theta)  \ , } \label{H:flux:approximate}
\end{equation}
where we have defined 
\begin{align}
k_{\text{eff}}^{(h)} & = \frac{8 \{k_1 k_2k_3\}^{(0)}}{\mathcal{M}^{(0)} } \ ; \label{gamma:0:definition} \\  
\Delta k_{\text{eff}}^{(h)}  & = \frac{ k_{\text{eff}}^{(h)} }{2} \left( \frac{\{ k_0 k_{-3} \}^{(1)}  }{  \{k_0 k_{-3} \}^{(0)} }  - \frac{\{k_1 k_3 \}^{(1)}}{\{ k_1 k_3 \}^{(0)}} \right) \ ,  \label{gamma:1:definition} \\
\delta \left(\Phi + C_h \right) & = \left[ (\Phi + C_h) - \int_0^{\pi}  (\Phi + C_h) K(\cos\theta) \ \sin \theta \ d  \theta \right] \ .
\end{align} 
{$k_{\text{eff}}^{(h)} c_{hp}^{\infty}>0$ is the typical scale  of the average proton consumption and production} and $\Delta k_{\text{eff}}^{(h)} c_{hp}^{\infty}$ \tl{the scale of the \emph{difference} between the rates at the pole and equator} due to variation of coating thickness over the surface.  
$\delta\left(\Phi + C_h\right)$ is the deviation of the perturbative fields from their surface average; which promotes/penalise the oxidation/reduction reactions. 
The proton flux $\bar{\mathcal{J}}_h$ is linear in $c_{hp}^{\infty}$ for low fuel concentration and the dependence weakens for high fuel concentration.
It is noteworthy that with uniform coating, $k_i = k_i^{(0)} \Rightarrow \Delta k_{\text{eff}}^{(h)} =0$ and the deviation fields vanish ($\Phi = 0 = C_i$). } \\
%$k_{\text{eff}}^{(h)} >0 $ is the typical scale  of the average proton consumption and production while $\Delta k_{\text{eff}}^{(h)} >0$ is the scale of the \emph{difference} between the rates at the pole and equator

%(\emph{Neutral solutes}) 
{The fluxes of neutral solutes from eqns. (\ref{o2:flux},\ref{hp:flux}) give 
\begin{align}
\bar{\mathcal{J}}_o(\theta)  \cong \  \frac{1}{2} \ k_{\text{eff}}^{(hp)} \bar{c}_{hp}(1,\theta) \ , \\
\bar{\mathcal{J}}_{hp}(\theta) \cong \  - \  k_{\text{eff}}^{(hp)}  \bar{c}_{hp}(1,\theta)  \ ,
\end{align}
%\begin{align}
% - \left. \frac{\partial C_o }{ \partial r} \right|_{r=1} & = \mathcal{J}_{o}(\theta) K(\cos \theta) \cong \quad \frac{1}{2} \left( \frac{ \mathcal{K}_{\text{eff}}^{(hp)}  a}{D_{o} c_{hp}^{\infty}} \right) K(\cos \theta) \ , \\
%- \left. \frac{\partial C_{hp} }{ \partial r} \right|_{r=1} & =  \mathcal{J}_{hp}(\theta) K(\cos \theta) \cong - \left( \frac{ \mathcal{K}_{\text{eff}}^{(hp)}  a}{D_{hp} c_{hp}^{\infty}} \right) K(\cos \theta) \ ,
%\end{align}
where the effective rate of hydrogen peroxide consumption is defined 
\begin{equation}
k_{\text{eff}}^{(hp)} = \frac{ 2}{\mathcal{M}^{(0)}} \{k_0 k_1 k_2 \}^{(0)} \bar{c}_{hp}(1,\theta) + \frac{1}{2} k_{\text{eff}}^{(h)} \ ,
\end{equation}
and the effective rate of proton consumption/desorption $k_{\text{eff}}^{(h)}$ is defined in equation (\ref{gamma:0:definition}). Note that $\bar{\mathcal{J}}_{hp}$ and $\bar{\mathcal{J}}_{o}$ are linear in $c_{hp}^{\infty}$ for low fuel ($c_{hp}^{\infty}$) concentraion, and exhibits Michaelis-Menten saturation for high fuel concentration.  }
% Note that $D_{hp} \mathcal{J}_{hp} + 2 D_o \mathcal{J}_o = 0$ and hence it suffices to solve for either of the fields to obtain the other.


\subsection{Reaction scheme 2}
%
\yhy{Alternatively, we may consider a different reaction scheme, with the same neutral pathway 
\begin{equation}
\mbox{Pt} +  2{\text{H}_2\text{O}_2} \ \overset{k_0}{\longrightarrow} \ \mbox{Pt}\left({\text{H}_2\text{O}_2} \right)  + {\text{H}_2\text{O}_2} \ \overset{k_1}{\rightarrow }\ \mbox{Pt}\left({\text{H}_2\text{O}_2} \right)_2 \ \overset{k_2}{\rightarrow} \  \mbox{Pt} + 2\text{H}_2\text{O} + \text{O}_2 \ ,  \label{h2o2:decomp:neutral2}
\end{equation} 
but having a different electrochemical pathway 
\begin{align}
& \mbox{Pt}\left({\text{H}_2\text{O}_2} \right) \quad \overset{k_3}{\longrightarrow} \quad \mbox{Pt} +  2\text{H}^+  + 2e^- + \text{O}_2 \ , \label{h2o2:decomp:oxidation}  \\ 
& \mbox{Pt}\left({\text{H}_2\text{O}_2} \right) + 2\text{H}^+  + 2e^- \quad \overset{k_4}{\longrightarrow} \quad \mbox{Pt} +  2\text{H}_2\text{O} \ .
\end{align} 
This is the reaction scheme commonly used in modeling the electrophoretic motion of the bimetallic nanorods~\cite{paxton2005motility,paxton2006chemical,sabass2012nonlinear}.
Similar to the first reaction scheme considered above, we enumerate the complexation kinetics of this reaction scheme in Fig.~\ref{reaction_scheme2}.
%
\begin{figure}
\begin{center}
\includegraphics[scale=.4]{reaction_schematic2}
\end{center}
\caption{(\textbf{Reaction scheme 2}): Schematic complexation kinetics of the Platinum catalyst with free ($0$'th state) Pt occupied with probability density $p_0$; first complex state $\text{Pt}(\text{H}_2\text{O}_2)$ occupied with probability density $p_1$, and the second complex state $\text{Pt}(\text{H}_2\text{O}_2)_2$ occupied with probability density $p_2$.} 
\label{reaction_scheme2}
\end{figure}
%
Here, solving for the fluxes $\bar{\mathcal{J}}_i$'s, in a similar manner to the calculations in the previous section, we obtain
%\begin{align}
%p_0 & =  \mathcal{M}^{-1} \, k_2 \left( k_1 \bar{c}_{hp} + k_3 + k_4 \bar{c}_{h}^2 \right) \  , \\
%p_1 & = \mathcal{M}^{-1} \, k_0 k_2 \bar{c}_{hp}  \ , \\
%p_2 & = \mathcal{M}^{-1}  \, k_0 k_1 \bar{c}_{hp}^2  \  , 
%\end{align} 
\begin{align}
\bar{\mathcal{J}}_{h}(\theta) & =  2 \, \mathcal{M}^{-1} \, k_0 k_2 \bar{c}_{hp} \left( k_3 - k_4 \bar{c}_{h}^2 \right) \, K(\cos \theta)   \  ,  \\
\bar{\mathcal{J}}_{hp}(\theta) & = - \mathcal{M}^{-1} \, k_0 k_2 \bar{c}_{hp} \left( 2k_1 \bar{c}_{hp} + k_3 + k_4 \bar{c}_{h}^2  \right) \,  K(\cos \theta)  \   , \\
\bar{\mathcal{J}}_o (\theta) & = \mathcal{M}^{-1} \, k_0 k_2 \bar{c}_{hp} \left( k_1 \bar{c}_{hp} + k_3 \right) \, K(\cos \theta)  \  ,
\end{align} 
where here
$\mathcal{M}  : = k_2 k_3 + \left( k_0 + k_1 \right)k_2 \bar{c}_{hp}  + k_2k_4\bar{c}_{h}^2 + k_0 k_1 \bar{c}_{hp}^2 \  .$
} \\


\par \noindent \textit{(Protons flux)} 
\yhy{Now, imposing the steady state constraint of $\oint \bar{\mathcal{J}}_{h}(\theta) d\cos\theta = 0$, and following the same calculation procedure as in the previous section (with $k_i = k_i^{(0)} + k_i^{(1)} \cos \theta$), we obtain the proton flux in equation (\ref{H:flux:approximate})
\begin{equation} 
\bar{\mathcal{J}}_h(\theta)  \cong \left[ \Delta k_{\text{eff}}^{(h)} \  \left( 1 - 2 \cos \theta \right)   - k_{\text{eff}}^{(h)} \ \delta \left(\Phi + C_h \right) \right] \bar{c}_{hp}^{\infty} \  K(\cos \theta)  \ ,  \label{H:flux:approximate2}
\end{equation}
where here we define 
\begin{align}
k_{\text{eff}}^{(h)} & = \frac{4 \{k_0 k_2k_3\}^{(0)}}{\mathcal{M}^{(0)} } \ ;  \qquad  
\Delta k_{\text{eff}}^{(h)}   = \frac{ k_{\text{eff}}^{(h)} }{2} \left( \frac{ k_4^{(1)}  }{ k_4^{(0)} }  - \frac{k_3^{(1)}}{k_3^{(0)}} \right) \ ,  \label{gamma:1:definition2}
\end{align}
while the deviation $\delta \left( \Phi + C_h \right) = \left[ ( \Phi + C_h) - \int_0^{\pi}  ( \Phi + C_h) K(\cos\theta) \ \sin \theta \ d  \theta \right]$ retain its previous definition. Finally, the same relation holds for $\varphi_s  = \varphi_s^{\ominus} - \ln 10 \ \mbox{pH}$ and the kinetically defined potential here is $\varphi_s^{\ominus} = - (1/2) \ln \left( k_3^{(0)}/k_4^{(0)} \right)$. Note that the two reaction schemes possess the same qualitative features --- the solute fluxes $\bar{\mathcal{J}}_i$'s retain the same functional dependence on the fuel concentraton $\bar{c}_{hp}$ and the reaction rates variation. }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
